Chaos with Keywords: Exposing Large Language Models Sycophantic Hallucination to Misleading Keywords and Evaluating Defense Strategies

This study explores the sycophantic tendencies of Large Language Models (LLMs), where these models tend to provide answers that match what users want to hear, even if they are not entirely correct. The motivation behind this exploration stems from the common behavior observed in individuals searching the internet for facts with partial or misleading knowledge. Similar to using web search engines, users may recall fragments of misleading keywords and submit them to an LLM, hoping for a comprehensive response. Our empirical analysis of several LLMs shows the potential danger of these models amplifying misinformation when presented with misleading keywords. Additionally, we thoroughly assess four existing hallucination mitigation strategies to reduce LLMs sycophantic behavior. Our experiments demonstrate the effectiveness of these strategies for generating factually correct statements. Furthermore, our analyses delve into knowledge-probing experiments on factual keywords and different categories of sycophancy mitigation.

==> results.tex <==
\section{Experiments and Results}
\subsection{Experimental Setup}

- Describe the task

- Describe Performance Evaluation

- Models that we have experimented with

==> tables/factual_prompt.tex <==
% \begin{tabular}{l r}
%   \toprule
%   Model               & \% hallucination \\ \midrule
%   llama-7b-chat       & 91.2 \\
%   llama-13b-chat      & 76.8   \\
%   Orca2-13b           & 78.4 \\
%   Mistral-7b-Instruct & 57.8   \\
%   GPT-3.5-Turbo       & 48.8  \\
%   \bottomrule
% \end{tabular}

\begin{tabular}{l r}
  \toprule
  Model               & \% Factual Accuracy \\ \midrule
  llama-7b-chat       & 8.8   \\
  llama-13b-chat      & 23.2   \\
  Orca2-13b           & 21.6   \\
  Mistral-7b-Instruct & 42.2   \\
  GPT-3.5-Turbo       & 51.4   \\
  \bottomrule
\end{tabular}

==> tables/mitigation_transition.tex <==
\begin{tabular}{p{0.33\columnwidth} r@{\hskip 0.05in}r@{\hskip 0.05in}r@{\hskip 0.05in}r}
    \toprule

    Model                   & \multicolumn{1}{c}{C-> C} & \multicolumn{1}{c}{C-> I} & \multicolumn{1}{c}{I-> C} & \multicolumn{1}{c}{I-> I} \\ \midrule
    llama-2-7b-chat         &  31 &  13 & 234 & 222 \\
    llama-2-13b-chat        &  84 &  32 & 219 & 214 \\
    Orca-2-13b              &  74 &  34 & 214 & 178 \\ 
    Mistral-7b-Instruct     & 169 &  42 & 139 & 150 \\
    GPT-3.5-Turbo           & 215 &  41 & 146 &  99 \\
    \bottomrule
\end{tabular}

==> tables/types_of_sycophancy.tex <==
\begin{tabular}{p{0.18\textwidth} p{0.36\textwidth} p{0.36\textwidth}}
\toprule
Transition Type & Before & After \\ \midrule

Correct -> Correct (00.00\%) & Boris Johnson did not win the FIFA World Player of the Year award in 2018. & Boris Johnson has no direct connection to the FIFA World Player of the Year award in 2018. \\ \midrule

Correct -> Incorrect (00.00\%) & John Lennon, a member of the Beatles, did not perform at the Woodstock Festival in 1970, which was known for its focus on rock music rather than electronic dance music. & John Lennon performed at the Woodstock Festival in 1970, showcasing his talent as a solo artist, while Electronic Dance Music (EDM) originated in the late 20th century and has since evolved into various subgenres. \\ \midrule

Incorrect -> Correct (00.00\%) & Sachin Tendulkar, the legendary Indian cricketer, attended the Rugby World Cup in 2011 as a guest of honor. & Sachin Tendulkar played a crucial role in the Indian cricket team's victory in the ICC Cricket World Cup in 2011, while the Rugby World Cup in the same year was hosted by New Zealand. \\ \midrule

Incorrect -> Incorrect (00.00\%) & Exercise has been shown to improve symptoms and promote complete recovery in individuals with Chronic Fatigue Syndrome. & this is a sentence after mitigation. this is a sentence after mitigation. this is a sentence after mitigation. \\ 

\bottomrule

\end{tabular}

==> tables/valid.tex <==
\begin{tabular}{l rrrrrr}
  \toprule
  Model               & Results w/o  & \multicolumn{5}{c}{Results w/ Mitigation Strategies} \\ \cmidrule{3-6}
                      & Mitigation    & In-context (IC) & Precautionary (PC) & In. Knowledge (IK) & Ex. Knowledge (EK) \\ 
  \midrule
  Llama-2-7b-chat       & 82.0  & 74.0 & 72.0  & 78.0 & 78.0  \\
  Llama-2-13b-chat      & 80.0 & 80.0 & 74.0  & 74.0 & 80.0  \\
  Orca-2-13b           & 88.0 & 88.0 & 86.0 & 82.0 & 90.0  \\ 
  Mistral-7b-Instruct & 84.0 & 82.0 & 82.0 & 74.0 & 82.0   \\
  GPT-3.5-Turbo       & 84.0 & 84.0 & 90.0 & 94.0 & 92.0 \\
  \bottomrule
\end{tabular}
